Self-Consistent Equation-guided Neural Networks for Censored Time-to-Event Data

In survival analysis, estimating the conditional survival function given predictors is often of interest. There is a growing trend in the development of deep learning methods for analyzing censored time-to-event data, especially when dealing with high-dimensional predictors that are complexly interrelated. Many existing deep learning approaches for estimating the conditional survival functions extend the Cox regression models by replacing the linear function of predictor effects by a shallow feed-forward neural network while maintaining the proportional hazards assumption. Their implementation can be computationally intensive due to the use of the full dataset at each iteration because the use of batch data may distort the at-risk set of the partial likelihood function. To overcome these limitations, we propose a novel deep learning approach to non-parametric estimation of the conditional survival functions using the generative adversarial networks leveraging self-consistent equations. The proposed method is model-free and does not require any parametric assumptions on the structure of the conditional survival function. We establish the convergence rate of our proposed estimator of the conditional survival function. In addition, we evaluate the performance of the proposed method through simulation studies and demonstrate its application on a real-world dataset.

==> myPKG.tex <==
\usepackage{graphicx}
\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage[italicdiff]{physics}
\usepackage[T1]{fontenc}
\usepackage{wrapfig}
\usepackage{lmodern,mathrsfs}
\usepackage[inline,shortlabels]{enumitem}
\usepackage[thinc]{esdiff}
\usepackage{mathtools}
\usepackage{microtype}
\usepackage{graphicx,wrapfig}
%\usepackage{subfigure}
\usepackage{booktabs}
\usepackage{comment}
\usepackage{relsize}
\usepackage{adjustbox}
\usepackage{float}
\usepackage{multirow}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage[numbers]{natbib}
\usepackage{epsfig,wrapfig,graphicx} 
\usepackage{threeparttable,multirow}
\usepackage{color}
%\usepackage{ulem}
\usepackage{adjustbox,booktabs,arydshln,multirow,url}
\usepackage{algorithm}
\usepackage{algorithmic}
% %\newcommand{\theHalgorithm}{\arabic{algorithm}}
%\usepackage{algorithm}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{subcaption}
\newenvironment{Boxedminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

%   \usepackage{hyperref}
% \usepackage{url}

% \usepackage{rotating,amsmath,amssymb,amsfonts,amsthm}
% \usepackage{epsfig,mathrsfs,natbib,color,graphics,comment}
% \usepackage{multirow}
% \usepackage{amsmath}
% \usepackage{mathtools}
% % if you use cleveref..
% %\usepackage[capitalize,noabbrev]{cleveref}
% \usepackage{graphicx}
% \usepackage{array,wrapfig,subfigure}
% \usepackage{hyperref}
% \usepackage{booktabs}
% % \def\boxit#1{\vbox{\hrule\hbox{\vrule\kern6pt \vbox{\kern6pt#1\kern5pt}
% % \kern6pt\vrule}\hrule}}
% % \renewcommand{\baselinestretch}{1.4}
% %\setlength{\oddsidemargin}{-0.15in}
% %\setlength{\topmargin}{-0.3in}  % 0.3 -0.1in
% %\setlength{\textheight}{9.3in}  % 9.1 9.3in
% %\setlength{\textwidth}{6.9in}
% \usepackage{geometry}
% % \geometry{a4paper,margin=1.0in}
% % \setlength{\parindent}{0.25in}
% % \setlength{\headsep}{0in}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% %\newcommand{\theHalgorithm}{\arabic{algorithm}}
% \usepackage[textsize=tiny]{todonotes}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % THEOREMS
% \newtheorem{theorem}{Theorem}[]
% \newtheorem{lemma}{Lemma}[]
% \newtheorem{definition}{Definition}[]
% \newtheorem{proposition}{Proposition}[]
% \newtheorem{corollary}{Corollary}[]
% \newtheorem{formula}{Formula}[]
% %\newtheorem{algorithm}{Algorithm}[]
% \newtheorem{remark}{Remark}[]
% \newtheorem{assumption}{Assumption}
% %%%%%%%%%%%%%%% newly defined notations %%%%%%%%%%%%%%%

% \usepackage{rotating,amsmath,amssymb,amsfonts,amsthm}
% \usepackage{epsfig,mathrsfs,natbib,color}
% \usepackage{graphicx,graphics,tikz}
% \usepackage{array,wrapfig}
% \usepackage{hyperref}
% \usepackage{booktabs,adjustbox,arydshln,multirow}
% %\usepackage{caption}
% \usepackage[utf8]{inputenc}  
% \usepackage[T1]{fontenc}     
% \usepackage{url}             
% \usepackage{nicefrac}   
% \usepackage{microtype}       
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage{tikz}

==> newfont.tex <==
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bX}{{\boldsymbol X}}
\newcommand{\bY}{{\boldsymbol Y}}
\newcommand{\mpi}{\cal \pi}
\newcommand{\by}{{\boldsymbol y}}
\newcommand{\bx}{{\boldsymbol x}} 
\newcommand{\bz}{{\boldsymbol z}}
\newcommand{\bZ}{{\boldsymbol Z}}
\newcommand{\bb}{{\boldsymbol b}}
\newcommand{\be}{{\boldsymbol e}}
\newcommand{\bw}{{\boldsymbol w}}
\newcommand{\bW}{{\boldsymbol W}}
\newcommand{\bM}{{\boldsymbol M}}
\newcommand{\bv}{{\boldsymbol v}}
\newcommand{\bs}{{\boldsymbol s}}
\newcommand{\bS}{{\boldsymbol S}}
\newcommand{\bA}{{\boldsymbol A}}
\newcommand{\bB}{{\boldsymbol B}}
\newcommand{\ba}{{\boldsymbol a}}
\newcommand{\bD}{{\boldsymbol D}}
\newcommand{\bE}{{\boldsymbol E}}
\newcommand{\bi}{{\boldsymbol i}}
\newcommand{\bc}{{\boldsymbol c}}
\newcommand{\bC}{{\boldsymbol C}}
\newcommand{\bK}{{\boldsymbol K}}
\newcommand{\bV}{{\boldsymbol V}}
\newcommand{\bG}{{\boldsymbol G}}
\newcommand{\bU}{{\boldsymbol U}}
\newcommand{\bu}{{\boldsymbol u}}
\newcommand{\bI}{{\boldsymbol I}}
\newcommand{\bJ}{{\boldsymbol J}}
\newcommand{\bQ}{{\boldsymbol Q}}
\newcommand{\mN}{\mathbb{N}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\mT}{\mathbb{T}}
\newcommand{\mI}{\mathbb{I}}
\newcommand{\mP}{\mathbb{P}}
\newcommand{\BX}{\mathbb{X}}
\newcommand{\BY}{\mathbb{Y}}
\newcommand{\BZ}{\mathbb{Z}}
\newcommand{\mB}{{\cal B}}
\newcommand{\mD}{{\cal D}}
\newcommand{\mF}{{\cal F}}
\newcommand{\mG}{{\cal G}}
\newcommand{\mbE}{{\mathbb{E}}}
\newcommand{\mE}{{\cal E}}
\newcommand{\tmE}{\widetilde{\cal E}}
\newcommand{\tbE}{\widetilde{\boldsymbol E}}
\newcommand{\me}{{\cal e}}
\newcommand{\mH}{{\cal H}}
\newcommand{\mJ}{{\cal J}}
\newcommand{\mK}{{\cal K}}
\newcommand{\mQ}{{\cal Q}}
\newcommand{\mX}{{\cal X}}
\newcommand{\mY}{{\cal Y}}
\newcommand{\mU}{{\cal U}}
\newcommand{\mM}{{\cal M}}
\newcommand{\mV}{{\cal V}}
\newcommand{\mL}{{\cal L}}
\newcommand{\mS}{{\cal S}}
\newcommand{\mZ}{\frak{Z}}
\newcommand{\mg}{{\cal g}}
\newcommand{\bxi}{{\boldsymbol \xi}}
\newcommand{\balpha}{{\boldsymbol \alpha}}
\newcommand{\bbeta}{{\boldsymbol \beta}}
\newcommand{\bgamma}{{\boldsymbol \gamma}}
\newcommand{\btheta}{{\boldsymbol \theta}}
\newcommand{\bTheta}{{\boldsymbol \Theta}}
\newcommand{\bthetaL}{{\btheta_{\Lambda}}}
\newcommand{\bvartheta}{{\boldsymbol \vartheta}}
\newcommand{\bepsilon}{{\boldsymbol \epsilon}}
\newcommand{\bvarepsilon}{{\boldsymbol \varepsilon}}
\newcommand{\bomega}{{\boldsymbol \omega}}
\newcommand{\bOmega}{{\boldsymbol \Omega}}
\newcommand{\bmu}{{\boldsymbol \mu}}
\newcommand{\seta}{\sigma_{\eta}}
\newcommand{\bsigma}{{\boldsymbol \sigma}}
\newcommand{\bSigma}{{\boldsymbol \Sigma}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\corr}{\mbox{Corr}}
\newcommand{\Var}{{\mbox{Var}}}
\newcommand{\cov}{{\mbox{Cov}}}
\newcommand{\diag}{{\mbox{diag}}}
\newcommand{\bYmis}{{\boldsymbol Y}_{{\rm mis}}}
\newcommand{\bYobs}{{\boldsymbol Y}^{{\rm obs}}}
\newcommand{\tbXmis}{{\tilde{\boldsymbol X}}^{{\rm  mis}}}
\newcommand{\tbxmis}{{\tilde{\boldsymbol x}}^{{\rm  mis}}}
\newcommand{\Zmis}{Z_{\rm mis}}
\newcommand{\Zobs}{Z_{\rm obs}}
\newcommand{\tXmis}{{\tilde{X}}^{{\rm  mis}}}
\newcommand{\txmis}{{\tilde{x}}^{{\rm  mis}}}
\newcommand{\Xmis}{X^{{\rm  mis}}}
\newcommand{\Xobs}{X^{{\rm  obs}}}
\newcommand{\bymis}{{\boldsymbol y}^{{\rm  mis}}}
\newcommand{\byobs}{{\boldsymbol y}^{{\rm  obs}}}
\newcommand{\ymis}{y^{{\rm  mis}}}
\newcommand{\yobs}{y^{{\rm  obs}}}
\newcommand{\Ymis}{Y^{{\rm  mis}}}
\newcommand{\Yobs}{Y^{{\rm  obs}}}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\bUmis}{{\boldsymbol U}_{{\rm mis}}}
% \newcommand{\bYmis}{{\boldsymbol Y}_{{\rm mis}}}
% \newcommand{\bYobs}{{\boldsymbol Y}_{{\rm obs}}}
% \newcommand{\tbXmis}{{\tilde{\boldsymbol X}}_{{\rm  mis}}}
% \newcommand{\tbxmis}{{\tilde{\boldsymbol x}}_{{\rm  mis}}}
\newcommand{\bXmis}{{\boldsymbol X}_{{\rm mis}}}
\newcommand{\bXobs}{{\boldsymbol X}_{{\rm obs}}}
\newcommand{\bZmis}{{\boldsymbol Z}_{{\rm mis}}}
\newcommand{\bZobs}{{\boldsymbol Z}_{{\rm obs}}}
%\newcommand{\tXmis}{{\tilde{X}}_{{\rm  mis}}}
%\newcommand{\txmis}{{\tilde{x}}_{{\rm  mis}}}
%\newcommand{\Xmis}{X_{{\rm  mis}}}
%\newcommand{\Xobs}{X_{{\rm  obs}}}
%\newcommand{\bymis}{{\boldsymbol y}_{{\rm  mis}}}
%\newcommand{\byobs}{{\boldsymbol y}_{{\rm  obs}}}
% \newcommand{\ymis}{y_{{\rm  mis}}}
% \newcommand{\yobs}{y_{{\rm  obs}}}
\newcommand{\red}{\textcolor{red}}
%\newenvironment{proof}{\trivlist\item[\hskip \labelsep{\sc Proof:}]}
% {\unskip\nobreak\ \lower.3ex\hbox{$\Box$}\endtrivlist}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{formula}{Formula}
%\newtheorem{algorithm}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{assump}{Assumption}
\newtheorem{assumpB}{Assumption}
\renewcommand\theassump{A\arabic{assump}}
\renewcommand\theassumpB{B\arabic{assumpB}}
\pagestyle{plain}
%\setcounter{secnumdepth}{5}
%\usepackage[numbers,sort]{natbib}
%\usepackage[authoryear]{natbib}
%\usepackage[numbers]{natbib}
%\bibliographystyle{asa}
%\bibliographystyle{listbib}

%%%%%%%%%%%% Journal definitions %%%%%%%%%%%%%%%%%%%%%%%%%
\def\AJE{{ American Journal of Epidemiology}}
\def\ANNALS{{ Annals of Statistics}}
\def\BIOK{{ Biometrika}}
\def\BMCS{{ Biometrics}}
\def\STATMED{{ Statistics in Medicine}}
\def\STATSCI{{ Statistical Science}}
\def\JSPI{{ Journal of Statistical Planning \& Inference}}
\def\JRSSB{{ Journal of the Royal Statistical Society, Series B}}
\def\COMMS{{ Communications in Statistics, Theory \& Methods}}
\def\JQT{{ Journal of Quality Technology}}
\def\TECH{{ Technometrics}}
\def\JASA{{ Journal of the American Statistical Association}}
\def\CSDA{{ Computational Statistics \& Data Analysis}}
\def\JCGS{{ Journal of Computational and Graphical Statistics}}
\def\JCB{{ Journal of Computational Biology}}
\def\BIOINF{{ Bioinformatics}}
\def\JAMA{{ Journal of the American Medical Association}}
\def\JNUTR{{ Journal of Nutrition}}
\def\LETTERS{{ Letters in Probability and Statistics}}
\def\JABES{{ Journal of Agricultural, Biological and
                      Environmental Statistics}}
\def\TECH{{ Technometrics}}
\def\COMMS{{ Communications in Statistics, Series A}}
\def\SCAN{{ Scandinavian Journal of Statistics}}
\def\PNAS{{ Proceedings of the National Academy of Sciences USA}}
\def\JMLR{{\it Journal of Machine Learning Research}}
\def\NEJM{{\it New England Journal of Medicine}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
